AlphaGAN: Fully Differentiable Architecture Search for Generative Adversarial Networks

Generative Adversarial Networks (GANs) are formulated as minimax game problems, whereby generators attempt to approach real data distributions by virtue of adversarial learning against discriminators. The intrinsic problem complexity poses the challenge to enhance the performance of generative networks. In this work, we aim to boost model learning from the perspective of network architectures, by incorporating recent progress on automated architecture search into GANs. To this end, we propose a fully differentiable search framework for generative adversarial networks, dubbed alphaGAN. The searching process is formalized as solving a bi-level minimax optimization problem, in which the outer-level objective aims for seeking a suitable network architecture towards pure Nash Equilibrium conditioned on the generator and the discriminator network parameters optimized with a traditional GAN loss in the inner level. The entire optimization performs a first-order method by alternately minimizing the two-level objective in a fully differentiable manner, enabling architecture search to be completed in an enormous search space. Extensive experiments on CIFAR-10 and STL-10 datasets show that our algorithm can obtain high-performing architectures only with 3-GPU hours on a single GPU in the search space comprised of approximate 2 ? 1011 possible configurations. We also provide a comprehensive analysis on the behavior of the searching process and the properties of searched architectures, which would benefit further research on architectures for generative models. Pretrained models and codes are available at https://github.com/yuesongtian/AlphaGAN.

==> Algorithm/algorithm_new.tex <==
\begin{algorithm}
    \caption{Detailed GANAS}
        \begin{algorithmic}
        \REQUIRE{
          \STATE Sample real data $x\sim\mathbb{P}_{r}$\;\\
          \STATE Sample latent variable $z\sim\mathbb{P}_{z}$\;\\}
        \ENSURE{
          \STATE Generator parameters $\theta$\;\\
          \STATE Generator operation weights $\alpha$\;\\}
        \end{algorithmic}
        \begin{algorithmic}[1] %每行显示行号
        \STATE initialize generator parameters $\omega_{G}$, generator architecture parameters $\alpha_{G}$, discriminator parameters $\omega_{D}$, Adam parameter $alpha$=0.0001, $beta_{1}$=0, $beta_{2}$=0.999.\\
        \FOR {$i$ of $search\_iterations$}
            \FOR {$k$ of $weight\_steps$}
                \FOR {$t$ of $n_{critic}$}
                    \STATE Sample a batch of real data ${x^{(i)}}\sim\mathbb{P}_{r}$ from training set;\\
                    \STATE Sample a batch of latent variables ${z^{(i)}}\sim\mathbb{P}_{z}$;\\
                    \STATE $L \leftarrow \sum_{i=1}^{m}{\rm ReLU}(1+D(G(z^{(i)})))+{\rm ReLU}(1-D(x^{(i)}));$
                    \STATE $\omega_{D} \leftarrow Adam(\nabla_{\omega_{D}}L,\omega_{D},alpha,beta_{1},beta_{2});$
                \ENDFOR
                \STATE Sample a batch of real data ${x^{(i)}}\sim\mathbb{P}_{r}$ from training set;\\
                \STATE Sample a batch of latent variables ${z^{(i)}}\sim\mathbb{P}_{z}$;\\
                \STATE $L \leftarrow \sum_{i=1}^{m}-{\rm ReLU}(1+D(G(z^{(i)})));$
                \STATE $\omega_{G} \leftarrow Adam(\nabla_{\omega_{G}}L,\omega_{G},alpha,beta_{1},beta_{2});$
            \ENDFOR
            \STATE
            $\overline{G}=G;$\\
            \STATE $\overline{D}=D;$\\
            \FOR {$k$ of $star\_steps$}
                \STATE Sample a batch of real data ${x^{(i)}}\sim\mathbb{P}_{r}$ from val set;\\
                \STATE Sample a batch of latent variables ${z^{(i)}}\sim\mathbb{P}_{z}$;\\
                \STATE $L \leftarrow \sum_{i=1}^{m}{\rm ReLU}(1+\overline{D}(G(z^{(i)})))+{\rm ReLU}(1-\overline{D}(x^{(i)}));$
                \STATE $\overline{\omega_{D}} \leftarrow Adam(\nabla_{\overline{\omega_{D}}}L,\overline{\omega_{D}},alpha,beta_{1},beta_{2});$
            \ENDFOR
            \FOR {$k$ of $star\_steps$}
                \STATE Sample a batch of real data ${x^{(i)}}\sim\mathbb{P}_{r}$ from val set;\\
                \STATE Sample a batch of latent variables ${z^{(i)}}\sim\mathbb{P}_{z}$;\\
                \STATE $L \leftarrow \sum_{i=1}^{m}-{\rm ReLU}(1+D(\overline{G}(z^{(i)})));$
                \STATE $\overline{\omega_{G}} \leftarrow Adam(\nabla_{\overline{\omega_{G}}}L,\overline{\omega_{G}},alpha,beta_{1},beta_{2});$
            \ENDFOR
            \FOR {$k$ of $arch\_steps$}
                \STATE Sample a batch of real data ${x^{(i)}}\sim\mathbb{P}_{r}$ from val set;\\
                \STATE Sample a batch of latent variables ${z^{(i)}}\sim\mathbb{P}_{z}$;\\
                \STATE $\rm{ Gap} \leftarrow \sum_{i=1}^{m}-{\rm ReLU}(1+\overline{D}(G(z^{(i)})))-{\rm ReLU}(1-\overline{D}(x^{(i)}))+{\rm ReLU}(1+D(\overline{G}(z^{(i)})))+{\rm ReLU}(1-D(x));$
                \STATE $\alpha_{G} \leftarrow Adam(\nabla_{\alpha_{G}}\rm{ Gap}, \alpha_{G},alpha,beta_{1},beta_{2});$
            \ENDFOR
        \ENDFOR
        \end{algorithmic}
\end{algorithm}

==> Algorithm/search_entire.tex <==
\begin{algorithm}
    \caption{Search the structure of GAN}
        \begin{algorithmic}[1] %每行显示行号
        \STATE initialize weight parameters and architecture parameters of $G (\omega_G,\alpha_{G})$, weight parameters of $D$ ($\omega_{D}$).\\
        \FOR {$i$ of $search\_iterations$}
            \FOR {$k$ of $weight\_steps$}
                \STATE train\_gan\_param($G$,$D$);\\
            \ENDFOR
            \STATE $\overline{G}=G$ and $\overline{D}=D$;\\
            \FOR {$k$ of $star\_steps$}
                \STATE approximate\_star($G$,$\overline{G}$,$D$,$\overline{D}$);\\            
            \ENDFOR
            \FOR {$k$ of $arch\_steps$}
                \STATE train\_gan\_arch($G$,$\overline{G}$,$D$,$\overline{D}$);\\
            \ENDFOR
        \ENDFOR
        \end{algorithmic}
\end{algorithm}

==> Algorithm/train_gan_arch.tex <==
\begin{algorithm}
    \caption{train\_gan\_arch}
        \begin{algorithmic}[1] %每行显示行号
        \STATE initialize $n\_critic$=5, batch size $m$=64, Adam parameter $alpha$=0.0001, $beta_{1}$=0.5, $beta_{2}$=0.999.\\
        \STATE Sample real data ${x^{(i)}}_{i=1}^{m}\sim\mathbb{P}_{r}$ from validation set and latent variables ${z^{(i)}}_{i=1}^{m}\sim\mathbb{P}_{z}$;\\
        \STATE ${\rm Gap} \leftarrow \sum_{i=1}^{m}-{\rm ReLU}(1+\overline{D}(G(z^{(i)})))-{\rm ReLU}(1-\overline{D}(x^{(i)}))+{\rm ReLU}(1+D(\overline{G}(z^{(i)})))+{\rm ReLU}(1-D(x));$
        \STATE $\alpha_{G} \leftarrow Adam(\nabla_{\alpha_{G}}{\rm Gap},\alpha_{G},alpha,beta_{1},beta_{2});$
        \end{algorithmic}
\end{algorithm}

==> Algorithm/train_gan_param.tex <==
\begin{algorithm}
    \caption{train\_gan\_param}
        \begin{algorithmic}[1] %每行显示行号
        \STATE initialize $n\_critic$=5, batch size $m$=64, Adam parameter $alpha$=0.0001, $beta_{1}$=0., $beta_{2}$=0.999.\\
        \FOR {$i$ of $n\_critic$}
            \STATE Sample real data ${x^{(i)}}_{i=1}^{m}\sim\mathbb{P}_{r}$ from training set and latent variables ${z^{(i)}}_{i=1}^{m}\sim\mathbb{P}_{z}$;\\
            \STATE $L \leftarrow \sum_{i=1}^{m}{\rm ReLU}(1+D(G(z^{(i)})))+{\rm ReLU}(1-D(x^{(i)}));$\\
            \STATE $\omega_{D} \leftarrow Adam(\nabla_{\omega_{D}}L,\omega_{D},alpha,beta_{1},beta_{2});$\\
        \ENDFOR
        \STATE Sample latent variables ${z^{(i)}}_{i=1}^{m}\sim\mathbb{P}_{z}$;\\
        \STATE $L \leftarrow \sum_{i=1}^{m}-D(G(z^{(i)}));$\\
        \STATE $\omega_{G} \leftarrow Adam(\nabla_{\omega_{G}}{\rm Gap},\omega_{G},alpha,beta_{1},beta_{2});$
        \end{algorithmic}
\end{algorithm}

==> table/ablation_study_large.tex <==
\begin{table}
  \caption{Ablation study on CIFAR-10 (large step size)}
  \label{Ablation study (large)}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{lllllllll}
    \toprule
    Name & Search D? & \multicolumn{3}{c}{obtain $\overline{G}$} & Gumbel-max? & Fix alphas? & IS & FID \\
    \cmidrule{3-5}
    & & update $\alpha_{G}$ & update $\omega_{G}$ & \tabincell{c}{update\\ $\alpha_{G}$ and $\omega_{G}$} \\
    \midrule
    Search D & $\checkmark$ & & $\checkmark$ & & $\times$ & $\times$ & $8.51\pm0.09$ & $18.07$\\
    w$\backslash$o search D & $\times$ & & $\checkmark$ & & $\times$ & $\times$ & $8.51\pm0.06$ & $11.38$\\
    \midrule
    Update $\omega_{G}$ & $\times$ & & $\checkmark$ & & $\times$ & $\times$ & $8.51\pm0.06$ & $11.38$\\
    Update $\alpha_{G}$ & $\times$ & $\checkmark$ & & & $\times$ & $\times$ & $7.06\pm0.06$ & $43.99$\\
    Update $\omega_{G}$ and $\alpha_{G}$ & $\times$ & & & $\checkmark$ & $\times$ & $\times$ & $8.43\pm0.11$ & $13.91$\\
    \midrule
    Gumbel-max & $\times$ & & $\checkmark$ & & $\checkmark$ & $\times$ & $8.48\pm0.10$ & $20.69$\\  
    w$\backslash$o Gumbel-max & $\times$ & & $\checkmark$ & & $\times$ & $\times$ & $8.51\pm0.06$ & $11.38$\\
    \midrule
    Fix alphas & $\times$ & & $\checkmark$ & & $\times$ & $\checkmark$ & $8.34\pm0.07$ & $15.49$\\
    w$\backslash$o fix alphas & $\times$ & & $\checkmark$ & & $\times$ & $\times$ & $8.51\pm0.06$ & $11.38$\\
    \bottomrule
  \end{tabular}}
\end{table}

==> table/ablation_study_small.tex <==
\begin{table}
  \caption{Ablation study on CIFAR-10 (small step size)}
  \label{Ablation study small}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{lllllllll}
    \toprule
    Name & Search D? & \multicolumn{3}{c}{obtain $\overline{G}$} & Gumbel-max? & Fix alphas? & IS & FID \\
    \cmidrule{3-5}
    & & update $\alpha_{G}$ & update $\omega_{G}$ & \tabincell{c}{update\\ $\alpha_{G}$ and $\omega_{G}$} \\
    \midrule
    Search D & $\checkmark$ & & $\checkmark$ & & $\times$ & $\times$ & $8.70\pm0.11$ & $15.56$\\
    w$\backslash$o search D & $\times$ & & $\checkmark$ & & $\times$ & $\times$ & $8.72\pm0.11$ & $12.86$\\
    \midrule
    Update $\omega_{G}$ & $\times$ & & $\checkmark$ & & $\times$ & $\times$ & $8.72\pm0.11$ & $12.86$\\
    Update $\alpha_{G}$ & $\times$ & $\checkmark$ & & & $\times$ & $\times$ & $8.45\pm0.09$ & $15.47$\\
    Update $\omega_{G}$ and $\alpha_{G}$ & $\times$ & & & $\checkmark$ & $\times$ & $\times$ & $8.18\pm0.11$ & $18.85$\\
    \midrule
    Gumbel-max & $\times$ & & $\checkmark$ & & $\checkmark$ & $\times$ & $8.56\pm0.06$ & $15.66$\\  
    w$\backslash$o Gumbel-max & $\times$ & & $\checkmark$ & & $\times$ & $\times$ & $8.72\pm0.11$ & $12.86$\\
    \midrule
    Fix alphas & $\times$ & & $\checkmark$ & & $\times$ & $\checkmark$ & $8.25\pm0.12$ & $19.07$\\
    w$\backslash$o fix alphas & $\times$ & & $\checkmark$ & & $\times$ & $\times$ & $8.72\pm0.11$ & $12.86$\\
    \bottomrule
  \end{tabular}}
\end{table}


==> table/ablation_study_summary.tex <==
\begin{table}
  \caption{Ablation studies on CIFAR-10}
  \label{Ablation study summary}
  \centering
  \resizebox{0.7\textwidth}{!}{
  \begin{tabular}{lllllll}
    \toprule
    Type & Search D? & \multicolumn{2}{c}{obtain $\overline{G}$} & IS & FID \\
    \cmidrule{3-4}
    & & update $\alpha_{G}$ & update $\omega_{G}$ \\
    \midrule
    \multirow{5}*{alphaGAN$_{(l)}$} & $\checkmark$ & $\times$ & $\checkmark$ & $8.51\pm0.09$ & $18.07$\\
     & $\times$ & $\times$ & $\checkmark$ & $8.51\pm0.06$ & $11.38$\\
    \cmidrule{2-6}
     & $\times$ & $\times$ & $\checkmark$ & $8.51\pm0.06$ & $11.38$\\
     & $\times$ & $\checkmark$ & $\times$ & $7.06\pm0.06$ & $43.99$\\
     & $\times$ & $\checkmark$ & $\checkmark$ & $8.43\pm0.11$ & $13.91$\\
    \midrule
    \multirow{5}*{alphaGAN$_{(s)}$} & $\checkmark$ & $\times$ & $\checkmark$ & $8.70\pm0.11$ & $15.56$\\
     & $\times$ & $\times$ & $\checkmark$ & $8.72\pm0.11$ & $12.86$\\
    \cmidrule{2-6}
     & $\times$ & $\times$ & $\checkmark$ & $8.72\pm0.11$ & $12.86$\\
     & $\times$ & $\checkmark$ & $\times$ & $8.45\pm0.09$ & $15.47$\\
     & $\times$ & $\checkmark$ & $\checkmark$ & $8.18\pm0.11$ & $18.85$\\
    \bottomrule
  \end{tabular}}
\end{table}


==> table/gumbelMax_WarmUp.tex <==
\begin{table}[b]
  \caption{Gumbel-max trick and Warm-up single.}
  \label{Gumbel-max trick and fix alphas}
  \centering
  \resizebox{0.5\textwidth}{!}{
  \begin{tabular}{llllll}
    \toprule
    Type & Name & Gumbel-max? & Fix alphas? & IS & FID \\
    \midrule
    \multirow{3}*{alphaGAN$_{(l)}$} & baseline & $\times$ & $\times$ & $8.88\pm0.12$ & $11.34$\\
     & Gumbel-max & $\checkmark$ & $\times$ & $8.48\pm0.10$ & $20.69$\\
     & Warm-up & $\times$ & $\checkmark$ & $8.34\pm0.07$ & $15.49$\\
    \midrule
    \multirow{3}*{alphaGAN$_{(s)}$} & baseline & $\times$ & $\times$ & $8.98\pm0.09$ & $10.35$\\
     & Gumbel-max & $\checkmark$ & $\times$ & $8.56\pm0.06$ & $15.66$\\
     & Warm-up & $\times$ & $\checkmark$ & $8.25\pm0.12$ & $19.07$\\
    \bottomrule
  \end{tabular}}
\end{table}
